Mechanics of micropillar confined thin film plasticity

Micropillar compression experiments probing size effects in confined plasticity of metal thin films, including the indirect imposition of 'canonical' simple shearing boundary conditions, show dramatically different responses in compression and shear of the film. The Mesoscale Field Dislocation Mechanics (MFDM) model is confronted with this set of experimental observations and shown to be capable of modeling such behavior, without any ad-hoc modification to the basic structure of the theory (including boundary conditions), or the use of extra fitting parameters. This is a required theoretical advance in the current state-of-the art of strain gradient plasticity models. It is also shown that significantly different inhomogeneous fields can display qualitatively similar size effect trends in overall agreement with the experimental results. The (plastic) Swift and (elastic) Poynting finite deformation effects are also demonstrated.

==> Pillar Size Effect Paper/temp-definitions.tex <==
\usepackage{amsmath}
\usepackage{amsbsy}
\usepackage{amssymb}
\usepackage{amscd}
\usepackage{amsfonts}

\newcommand{\R}{\mathbb R}
\newcommand{\N}{\mathbb N}
\newcommand{\Z}{\mathbb{Z}}

\newcommand{\bs}{\boldsymbol}
\newcommand{\la}{\boldsymbol{\lambda}}
\newcommand{\Curl}{\textit{curl}\:}
\newcommand{\Grad}{\textit{grad}\:}

\newcommand{\bfa}{{\mathbold a}}
\newcommand{\bfb}{{\mathbold b}}
\newcommand{\bfc}{{\mathbold c}}
\newcommand{\bfd}{{\mathbold d}}
\newcommand{\bfe}{{\mathbold e}}
\newcommand{\bff}{{\mathbold f}}
\newcommand{\bfg}{{\mathbold g}}
\newcommand{\bfh}{{\mathbold h}}
\newcommand{\bfi}{{\mathbold i}}
\newcommand{\bfj}{{\mathbold j}}
\newcommand{\bfk}{{\mathbold k}}
\newcommand{\bfl}{{\mathbold l}}
\newcommand{\bfm}{{\mathbold m}}
\newcommand{\bfn}{{\mathbold n}}
\newcommand{\bfo}{{\mathbold o}}
\newcommand{\bfp}{{\mathbold p}}
\newcommand{\bfq}{{\mathbold q}}
\newcommand{\bfr}{{\mathbold r}}
\newcommand{\bfs}{{\mathbold s}}
\newcommand{\bft}{{\mathbold t}}
\newcommand{\bfu}{{\mathbold u}}
\newcommand{\bfv}{{\mathbold v}}
\newcommand{\bfw}{{\mathbold w}}
\newcommand{\bfx}{{\mathbold x}}
\newcommand{\bfy}{{\mathbold y}}
\newcommand{\bfz}{{\mathbold z}}

\newcommand{\bfA}{{\mathbold A}}
\newcommand{\bfB}{{\mathbold B}}
\newcommand{\bfC}{{\mathbold C}}
\newcommand{\bfD}{{\mathbold D}}
\newcommand{\bfE}{{\mathbold E}}
\newcommand{\bfF}{{\mathbold F}}
\newcommand{\bfG}{{\mathbold G}}
\newcommand{\bfH}{{\mathbold H}}
\newcommand{\bfI}{{\mathbold I}}
\newcommand{\bfJ}{{\mathbold J}}
\newcommand{\bfK}{{\mathbold K}}
\newcommand{\bfL}{{\mathbold L}}
\newcommand{\bfM}{{\mathbold M}}
\newcommand{\bfN}{{\mathbold N}}
\newcommand{\bfP}{{\mathbold P}}
\newcommand{\bfQ}{{\mathbold Q}}
\newcommand{\bfR}{{\mathbold R}}
\newcommand{\bfS}{{\mathbold S}}
\newcommand{\bfT}{{\mathbold T}}
\newcommand{\bfU}{{\mathbold U}}
\newcommand{\bfV}{{\mathbold V}}
\newcommand{\bfW}{{\mathbold W}}
\newcommand{\bfX}{{\mathbold X}}
\newcommand{\bfY}{{\mathbold Y}}
\newcommand{\bfZ}{{\mathbold Z}}

\newcommand{\tbfy}{{\tilde{\bfy}}}
\newcommand{\vphi}{{\varphi}}
\newcommand{\eps}{{\varepsilon}}
\newcommand{\Nhat}{\hat{\mbox{\tiny {\bf N}}}}
\newcommand{\ehat}{\hat{\bfe}}
\newcommand{\nhat}{\hat{\bfn}}
\newcommand{\uhat}{\hat{\bfu}}
\newcommand{\phihat}{\hat{\varphi}}
\newcommand{\adj}{{\mbox{adj }}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqs}{\begin{eqnarray}}
\newcommand{\eeqs}{\end{eqnarray}}
\newcommand{\beql}{\begin{equation} \label}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\del}{\partial}

\newcommand{\calA}{{\cal A}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calI}{{\cal I}}
\newcommand{\calJ}{{\cal J}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calV}{{\cal V}}

\newcommand{\sint}{-\hspace{-4mm}\int} % slashed integral, math
\newcommand{\ssint}{-\hspace{-3mm}\int} % slashed integral, text
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{corollary}{Corollary}[section]

\newcommand{\bfchi}{\mathbold{\chi}}
\newcommand{\bfdelta}{\mathbold{\delta}}
\newcommand{\bfsigma}{\mathbold{\sigma}}
\newcommand{\bfepsilon}{\mathbold{\epsilon}}
\newcommand{\bfnu}{\mathbold{\nu}}
\newcommand{\bfalpha}{\mathbold{\alpha}}
\newcommand{\bfomega}{\mathbold{\omega}}
\newcommand{\bfbeta}{\mathbold{\beta}}
\newcommand{\bfvphi}{\mathbold{\varphi}}
\newcommand{\bfveps}{\mathbold{\varepsilon}}
\newcommand{\bfPi}{\mathbold{\Pi}}

\newcommand{\bfLambda}{\mathbold{\Lambda}}
\newcommand{\bfGamma}{\mathbold{\Gamma}}
\newcommand{\bfOmega}{\mathbold{\Omega}}
\newcommand{\bfTheta}{\mathbold{\Theta}}
\newcommand{\bfSigma}{\mathbold{\Sigma}}
\newcommand{\bfDelta}{\mathbold{\Delta}}

\newcommand{\bfzero}{\mathbf{0}}
\newcommand{\erf}{\mathop{\rm erf}\nolimits}
\newcommand{\erfc}{\mathop{\rm erfc}\nolimits}
\newcommand{\grad}{\mathop{\rm grad}\nolimits}
\newcommand{\divergence}{\mathop{\rm div}\nolimits}
\newcommand{\curl}{\mathop{\rm curl}\nolimits}
\newcommand{\trace}{\mathop{\rm tr}\nolimits}
\newcommand{\GCD}{\mathop{\rm GCD}\nolimits}

\newcommand{\parderiv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\deriv}[2]{\frac{d #1}{d #2}}
\newcommand{\bsl}{\backslash}
\newcommand{\veps}{\varepsilon}


\newenvironment{rcases}
  {\left.\begin{aligned}}
  {\end{aligned}\right\rbrace}
%%

\newcommand{\p}{\partial}


